Digital Nudging with Recommender Systems: Survey and Future Directions

Recommender systems are nowadays a pervasive part of our online user experience, where they either serve as information filters or provide us with suggestions for additionally relevant content. These systems thereby influence which information is easily accessible to us and thus affect our decision-making processes though the automated selection and ranking of the presented content. Automated recommendations can therefore be seen as digital nudges, because they determine different aspects of the choice architecture for users. In this work, we examine the relationship between digital nudging and recommender systems, topics that so far were mostly investigated in isolation. Through a systematic literature search, we first identified 87 nudging mechanisms, which we categorize in a novel taxonomy. A subsequent analysis then shows that only a small part of these nudging mechanisms was previously investigated in the context of recommender systems. This indicates that there is a huge potential to develop future recommender systems that leverage the power of digital nudging in order to influence the decision-making of users. In this work, we therefore outline potential ways of integrating nudging mechanisms into recommender systems.

==> list_implemented_nudges.tex <==
% Changing the overall size of the table
\small

\begin{longtable}[c]{p{5cm}p{2cm}p{6cm}}
	\hline
	\textbf{Nudge} & \textbf{Applied?} & \textbf{Possible implementation} \\
	\endfirsthead
	%
	\hline
	\multicolumn{3}{c}%
	{{\bfseries Table \thetable\ continued from previous page}} \\
	\textbf{Nudge} & \textbf{Applied?} & \textbf{Possible implementation} \\
	\endhead
	%
	\hline
	Increase salience of incentives &  & Increasing the visibility of the incentives of a recommender (e.g. the benefits of finding an item) \\
	\hline
	Providing Feedback & Yes & Providing the user feedback on their choices or why a certain item is provided. \\
	\hline
	Setting Defaults (Status Quo Bias) & Yes & Preselecting the best choice for a user. \\
	\hline
	Understanding Mapping &  & Explaining to the user why a certain recommendation has been provided - using analogies \\
	\hline
	Expecting Error &  & Expecting the user to make mistakes in the recommendation process and providing a safety net. Telling the user beforehand what mistakes usually happen and how to work around this. Having useful error pages. \\
	\hline
	Structure Complex Choices & Yes & Listing all the attributes of all the alternatives and letting people make trade-offs when necessary. \\
	\hline
	Anchoring and Adjusting &  & Anchoring a selection of recommendations with another item. (E.g. setting a higher/lower anchor to steer the user's behaviour) \\
	\hline
	Customized Information (Tailoring) &  & Providing (seemingly) personalized information (e.g. "Because of certain behaviour this option should be most fitting to you", "Based on your personal preferences..." \\
	\hline
	Decision Staging (Tunneling) &  & Giving users the choice to manage the criteria by which they are comparing their options. \\
	\hline
	Availability &  & Making information seem generally more available (e.g. by implying that a certain situation happens very often like a dinner with friends) \\
	\hline
	Framing & Yes & Framing an option/selection to be better or poorer by creating a scenario or situation. \\
	\hline
	Informing & Yes & Simply by providing more information to the options. Could be by having "More information". Can also work into the opposite direction by reducing the available information on a certain item. \\
	\hline
	Limited Time Window &  & Presenting an option/item as a limited time offer. \\
	\hline
	Representativeness &  & Using stereotypes to steer the expectiations of certain items (using brand names, countries, racial stereotypes) \\
	\hline
	Precommitment Strategy &  & Letting a user decide on a goal before they actually get their recommendations (Eat healthier) and then to possibly remind them that a certain option is (not) alligning to that goal \\
	\hline
	Priming & Yes & Using stereotypes to steer the expectiations of certain items (using brand names, countries, racial stereotypes) \\
	\hline
	Reminders & Yes & Using reminders to finish their recommendation process (you have not yet found a movie you like?). Reminding them of the benefits of having a new car. \\
	\hline
	Simplification (Reduction) &  & Simplifying the process of finding a recommended item (Google's Feeling Lucky option). E.g. making automated recommendations/providing recommendations based on other criteria which are easily available. Just the genre/category for example. \\
	\hline
	Social Influence (Social Comparison) &  & Stating what most other people selected (User's favourite) \\
	\hline
	Warning &  & Warning the user of an action that might not benefit them (Selecting an unealthy option on a menu) \\
	\hline
	Partition of Options/Categories &  & Making categories of the provided elements (different lists). Steering people to select an item out of each list or does the experience of lists have an effect on the user experience \\
	\hline
	Providing an Explanation &  & Providing explanations to why the RS choose a certain option for the user. \\
	\hline
	Changing scale &  & Changing the scale of certain attributes of an item to make them appear bigger/smaller in comparison. \\
	\hline
	Explicitly Mapping &  & Making the correlation of options to their consequences more visible - How costs will unfold if certain options are chosen \\
	\hline
	Increasing Ease and Convenience &  & Making certain features of the RS more easy to use than others. Finding options that are healthier is more easy than finding unhealthy options. \\
	\hline
	Disclosure &  & Same as explicitly mapping. Making sure that every aspect is provided to a pricing model in comparison to some options that do not. \\
	\hline
	Eliciting Implementation Intentions &  & Stating what the user probably intends to do by using the RS. Like: So you want to eat healthier? These are some good options. \\
	\hline
	Informing people of the nature and consequences of their own past choices &  & Through implicit or explicit saving of user's beahviour the RS could tell the user that they tend to select many options of a certain category and might want to change that beahviour. Could say that they did spend a lot of money on shoes in the last year and maybe search for cheaper options. \\
	\hline
	Optimism and Overconfidence &  &  \\
	\hline
	Loss Aversion &  & Emphasizing the loss of certain options in comparison to others. Providing many items in a comparison and concentrating on the loss if not the best option is chosen. \\
	\hline
	Temptation (Greed, short-term reward) &  & Emphasizing the immediate benefits of certain options. \\
	\hline
	Self-control strategies (Self-Commitment) &  & Providing a mechanism which helps users to overcome their "habits". E.g. using the RS as a coach or a system that helps them fulfill their goal. \\
	\hline
	Following the herd (Social norms) &  & Text like: "Other people also liked". Users will be drawn towards what another people did. \\
	\hline
	Spotlight Effect (Raising the visibility of user's action) &  & Text like: "Other people will see the decisions you made", "Comments will be visible for all other users" \\
	\hline
	Salience & Yes & Simply increasing the visibility of any option. E.g. using colours \\
	\hline
	Consequences (Social norms) & Yes & "Your actions will have an impact on the experience of others" (Linked to spotlight effect sometimes) \\
	\hline
	Make internal/external information visible & Yes & Presenting the algorithm by which an option was chosen. Showing what data was used to make the recommendation. \\
	\hline
	Refering to opinion leader &  & Presenting an instance that is used as an opinion leader (website, doctor, athlete, etc.) \\
	\hline
	Prompted Choice &  & Making the user actively choose attributes/characteristics for an option \\
	\hline
	Increase/Decrease physical effort &  & Only possible for certain situations which involve a physical step (E.g. signing a contract). It would emphasize that a certain recommendation does not need that physical step or rather that it reduces the work on the side of the user. Scrolling. \\
	\hline
	Increase/Decrease financial effort &  & By changing the perceived costs of an item (without actually changing the costs). This can be done by splitting the costs etc. \\
	\hline
	Support public commitment & Yes & Making the user commit in a public scenario for other users to see. (Eat healthier) \\
	\hline
	"Micro-Incentives" &  & Charging the user 1 cent additionally for unwanted options. E.g. unhealthy options. \\
	\hline
	Public (Social) &  & Making the user commit in a public scenario for other users to see. (Eat healthier) \\
	\hline
	Just-in-time & Yes & Make recommendations for the user when they are appropriate. E.g. user is already active on the phone or computer and not when the user has set the phone to silent. \\
	\hline
	Situated & Yes & Make recommendations when the situation is fitting. E.g. user is searching for recipes or the time frame would suggest to eat. \\
	\hline
	Apprehensive & Yes &  \\
	\hline
	Automated & Yes & Automatically make recommendations for the user. \\
	\hline
	Tutorial & Yes & Present the user how to generate recommendations with an example. \\
	\hline
	Positive & Yes & Commending the user for using the recommender/choosing one of the recommendations. \\
	\hline
	Making information visible &  & Presenting the algorithm by which an option was chosen. Showing what data was used to make the recommendation. \\
	\hline
	Translate information &  &  \\
	\hline
	Provide social reference point &  &  \\
	\hline
	Change option-related effort &  &  \\
	\hline
	Change range or composition of options &  &  \\
	\hline
	Facilitate commitment &  &  \\
	\hline
	Change option consequences &  &  \\
	\hline
	Simplifiying active choosing &  & Asking people whether they want to choose or instead to rely on a default rule. Additionally improving the active choosing by providing help/reference. \\
	\hline
	Enhancing or influencing active choosing &  & Asking people to choose but influencing the situation by using other nudges. \\
	\hline
	Navigability of Contexts &  & Improving/Worsen the navigability of options and contexts of a recommendation. \\
	\hline
	Ordering effects & Yes & Ordering the items of a recommender. \\
	\hline
	Speed bumps &  & Creating speed bumps in the process of generating recommendations so the user has to think about certain attributes. Having specific moments in the procedure to slow down. \\
	\hline
	Automatic enrollment (Opt-out policies) &  & Automatically enrolling the user into providing the most healthy/best fitting results. The user then has to opt-out. (E.g. showing the vegan option as the first item always. \\
	\hline
	Visuals & Yes & Using visuals to draw the attention towards specific options OR using visuals to make options less interesting. \\
	\hline
	Decrease Vagueness and Ambiguity &  & By making statements more accurate and clear a certain recommendation can be deemed more interesting. \\
	\hline
	Attracting/Reducing Attention &  & Any form of attracting/reducing the attention of an option is encompassed i this. E.g. design of the decision. \\
	\hline
	Moral Suasion &  & Persuading the user that they actually responsibility in the situation. This could be done through entailing some sort of later use of the data generated. Even if it is only for the later recommendations of the user. \\
	\hline
	Checklists &  & Using checklists to structure the recommendation procedure (Making steps visible to the user) \\
	\hline
	Reducing paperwork &  & Emphasizing the reduction of paperwork when selecting an option provided by the RS. E.g. if a insurance is bought or any other e-commerce item which would possibly need the user to act on paper. \\
	\hline
	Giving comparative information &  & Providing different viewpoints on a recommendation. E.g. providing comparative data in a designated window. \\
	\hline
	Structure of Evaluation &  & Let users evaluate the items jointly rather than seperately so that they actually rate all the items. \\
	\hline
	Visible Goals &  & Making goals visible as such. E.g. end of recommendation process, result of the recommendation process. \\
	\hline
	Argentum Ad Populum & Yes &  \\
	\hline
	Group-Ad Populum & Yes &  \\
	\hline
	Hyperbolic Discounting & Yes & Financing and deferred payment for products on e-commerce websites, decoupling the purchase from the payment, lowering the purchase barrier, and shortening the decision-making process \\
	Decoupling &  &  \\
	\hline
	Mental Accounting &  &  \\
	\hline
	Attentional Collapse &  &  \\
	\hline
	Messenger Effect &  &  \\
	\hline
	Image Motivation &  &  \\
	\hline
	Intertemporal Choice &  &  \\
	\hline
	Endowment Effect &  &  \\
	\hline
	Hiding &  & Making undesirable options harder to reach. \\
	\hline
	Suggesting alternatives & Yes & Drawing attention to options that might have not been considered - "Have you also looked at...?" \\
	\hline
	Throttling mindless activity &  & Giving the user the possibility to change their mind (fitting for situation). E.g. After purchasing they have the possibility to change their mind for an additional 10 seconds. \\
	\hline
	Creating friction &  & Changing the behaviour of the user with as little intrusion as possible. Depends on the specific field but still. \\
	\hline
	Providing multiple viewpoints &  & Similar to providing comparative information but now providing this information unbiased. \\
	\hline
	Decoy effect & Yes  & Adding an inferior alternative to make the other options seem better. \\
	\hline
	Biasing the memory of past experiences &  & By making the end of a task seem different (E.g. changing the speed of a progress bar, reducing workload at the end) \\
	\hline
	Placebos &  &  \\
	\hline
	Deceiptive visualizations &  & Creating optical illusions that alter people's perception and judgements. E.g. making an option seem better in comparison to others. Use of colours or size. \\
	\hline
	Invoking feelings of reciprocity &  & Offering something small in return for feelings of reciprocity. E.g. giving the user something small like a free wallpaper/pin/other small benefit. \\
	\hline
	Make resources scarce &  & Announcing limited seats at future events increses the probability of people commiting. \\
	\hline
	Reducing the distance &  &  \\
	\hline
	Instigating empathy &  & E.g. providing an animal that changes its state based on the behaviour of a user. \\
	\caption{Nudges implemented in recommender systems}
\end{longtable}

==> list_nudges.tex <==
% Changing the overall size of the table
\small

\begin{longtable}[c]{@{}p{5cm}p{8cm}@{}}
	\toprule
	\textbf{Name} &
	\multicolumn{1}{l}{\textbf{Description}} \\
	\endfirsthead
	%
	\multicolumn{2}{c}%
	{{\bfseries Table \thetable\ continued from previous page}} \\
	\toprule
	\textbf{Name} &
	\multicolumn{1}{l}{\textbf{Description}} \\
	\endhead
	%
	Increase salience of   incentives &
	Making   incentives more salient to increase their effectiveness. \\
	\hline
	Providing   Feedback &
	Providing   users with feedback when they are doing well or making mistakes \\
	\hline
	Setting Defaults (Status Quo Bias) &
	Preselecting   options by setting default options \\
	\hline
	Understanding Mapping &
	Mapping   information that is difficult to evaluate to familiar evaluation schemes \\
	\hline
	Expecting Error &
	\begin{tabular}[c]{@{}l@{}}Expecting   users to make errors and being as\\      forgiving as possible\end{tabular} \\
	\hline
	Structure Complex Choices &
	Listing   all the attributes of all the alternatives and letting people make trade-offs   when necessary \\
	\hline
	Anchoring and Adjusting &
	In   simple terms an anchor is a clue, or cue, or a pointer, or a starting point,   (whose scale/quality we think we know reasonably reliably) which can be   adjusted to help us to estimate an answer. \\
	\hline
	Customized Information (Tailoring) &
	Tailoring   the provided alternatives/attributes to reduce cognitive overload \\
	\hline
	Decision Staging (Tunneling) &
	When   people make complex or long decisions, such as buying a car, they tend to   successively explore their options. This includes what information to focus   on, as well as choices between attributes and alternatives. For example, when   people narrow down their options, they often tend to screen alternatives on   the basis of a subset of attributes and then compare alternatives. \\
	\hline
	Availability &
	Visibility,   or how commonly something is perceived to arise in a general sense, which   significantly influences people's assessment of how likely it is to arise in   a personal sense. \\
	\hline
	Framing &
	Language   is immensely flexible. Something which is a good possibility/option may   always be described or 'framed' as a poor one, and vice-versa. \\
	\hline
	Informing &
	Providing   information to the user. \\
	\hline
	Limited Time Window &
	One   way to present scarcity of an object. \\
	\hline
	Representativeness &
	Expecting   a member of a group to have certain characteristics without having actual   information about that individual. \\
	\hline
	Precommitment Strategy &
	People   commiting to a certain course of actions ( e.g. defining a goal) \\
	\hline
	Priming &
	Anchoring   or focalism is a cognitive bias where an individual depends too heavily on an   initial piece of information offered (considered to be the   "anchor") when making decisions. \\
	\hline
	Reminders &
	Setting   reminders for overdue bills and coming obligations or appointments (form of   email, text, etc.) \\
	\hline
	Simplification (Reduction) &
	An   alternative way of making existing information more helpful to decision   makers is simplification, that is, reducing the burden of cognitive effort   necessary to process the information available and increase its usefulness in   the decision making process. \\
	\hline
	Social Influence (Social Comparison) &
	Emphasizing   what most people do, e.g., "most people plan to vote" or "most   people pay their taxes on time" or "nine out of ten hotel guests   reuse their towels" \\
	\hline
	Warning &
	Warnings   in the form of grapics or otherwise \\
	\hline
	Partition of Options/Categories &
	A   choice architect can tactically arrange the respective categories or   allocation alternatives, such as segregating healthy options into more   diverse categories. \\
	\hline
	Providing an Explanation &
	Providing   additional information in order for the situation to be more understandable. \\
	\hline
	Changing scale &
	Expanding   the denominator makes the numerators larger and makes the differences between   alternatives appear larger, leading these expanded attributes to receive more   weight in choice. \\
	\hline
	Explicitly Mapping &
	There   is a benefit in explicitly mapping an attribute to its consequences for other   objectives (e.g. costs, benefits) \\
	\hline
	Increasing Ease and Convenience &
	Making   low-cost options or healthy foods visible. Emphasis lies on the visibility   and accessability \\
	\hline
	Disclosure &
	Disclosing   related information (Full cost of certain credit cards) \\
	\hline
	Eliciting Implementation Intentions &
	People   are more likely to engage in activity if someone elicits their implementation   intentions (e.g. "do you plan to vote?") \\
	\hline
	Informing people of the nature and consequences of their own   past choices &
	Specific   case of "Informing" {[}N012{]}. Institutions often have a lot of   information about people's own past choices. If these individuals obtain that   information they can shift their behavior. \\
	\hline
	Optimism and Overconfidence &
	This   is the tendency to under-estimate costs, timescales, challenges, and to   over-estimate rewards and the ease of unknown things. \\
	\hline
	Loss Aversion &
	The   disutility of giving up an object is greater than the utility associated with   acquiring it. (see also Sunk cost effects and endowment effect). \\
	\hline
	Temptation (Greed, short-term reward) &
	People   are generally and naturally attracted to options which offer quick appealing   reward. \\
	\hline
	Self-control strategies (Self-Commitment) &
	People   are often aware that they have some 'heuristic' weaknesses, which they might   regard as 'bad habits', or simply 'weaknesses'). Supporting them in helping   fulfil their plan is a possible implementation. \\
	\hline
	Following the herd (Social norms) &
	Group   of nudges corresponding to Social Norms \\
	\hline
	Spotlight Effect (Raising the visibility of user's action) &
	This   is the tendency for people to over-estimate the visibility/significance of   their own decisions and actions, which Thaler and Sunstein call the   'spotlight effect'. \\
	\hline
	Salience &
	The   act of making something more salient (attribute, option, etc.) \\
	\hline
	Consequences (Social norms) &
	Consequences   are occuring for other colleagues if a certain activity is performed   (Presented as information) \\
	\hline
	Make internal/external information visible &
	Similar   to "Explicitly mapping" and "Providing feedback", this   Nudge provides all necessary information needed for a decision. \\
	\hline
	Refering to opinion leader &
	Highly   valued, respected messengers (e.g., experts or role models) can influence   opinions and behavior. \\
	\hline
	Prompted Choice &
	Prompted   choice avoids the status quo bias or default effects because of inertia or   assumed recommendations. However, enforcing active choice and deliberation   may give cognitive biases more influence because of greater reflection. In   short: Making users actively make a decision. \\
	\hline
	Increase/Decrease physical effort &
	Making   an apple easier to grasp than less healthy alternatives is discussed as an   example for promoting healthy choices in a situation where hunger or appetite   depletes self-control, leading to regrettable decisions. \\
	\hline
	Increase/Decrease financial effort &
	Independent   of the actual amount in question, people perceive the realization of   financial transactions as more or less costly. Choice architects can   intervene to change the factors determining this perception of financial   effort. Final price remains unchanged! Examples include postponing costs to   the future without changin the actual final costs. \\
	\hline
	Support public commitment &
	Commitments   can be made in front of other people, thus introducing another “supervisor”   in addition to the self. Publicly committing to a behavior (working out) or   to refrain from a behavior (smoking) creates external pressure and possibly   negative consequences in case of breaking the commitment. See   "Self-control strategies". \\
	\hline
	"Micro-Incentives" &
	Changes   of the consequences of decision options that are insignificant from a   rational choice perspective (e.g., providing an improbable chance of winning   a lottery or requiring middle class shoppers to pay five cents for a shopping   bag \\
	\hline
	Public (Social) &
	See   "Support public commitment" \\
	\hline
	Just-in-time &
	Make   recommendations/Draw attention when an action is appropriate \\
	\hline
	Situated &
	Make   suggestions where the practive is applicable \\
	\hline
	Apprehensive &
	Providing   multiple locations where activities can be applied \\
	\hline
	Automated &
	Perform   actions for users and present output \\
	\hline
	Tutorial &
	Show   how to complete a practice \\
	\hline
	Positive &
	Commend   users to encouraged action adoption \\
	\hline
	Making information visible &
	See   "Making internal/external information visible" \\
	\hline
	Translate information &
	Group   of nudges: See "Mapping" \\
	\hline
	Provide   social reference point &
	Group   of nudges: See "Social" \\
	\hline
	Change   option-related effort &
	Group   of nudges: See "effort" \\
	\hline
	Change   range or composition of options &
	Group   of nudges: See "Scale" and "Partition" \\
	\hline
	Facilitate   commitment &
	Group   of nudges: See "Commitment" \\
	\hline
	Change   option consequences &
	Group   of nudges: E.g. micro-incentives \\
	\hline
	Simplifiying   active choosing &
	Asking   people whether they want to choose or instead to rely on a default rule \\
	\hline
	Enhancing   or influencing active choosing &
	Asking   people to choose but using order effects or loss aversion to influence   choices; alternatively, enlisting authority to influence people \\
	\hline
	Navigability   of Contexts &
	Making   contexts or policies easily navigable, with pointers and guides \\
	\hline
	Ordering effects &
	What   people see first on a website or in a room; asking people to sign forms on   the first page. (Order of elements) \\
	\hline
	Speed bumps &
	Providing   literal or figurative speed bumps or cooling-off periods (as for waiving   rights) \\
	\hline
	Automatic enrollment (Opt-out policies) &
	Offering   automatic enrollment with precommitment \\
	\hline
	Visuals &
	Using   visual effects, colors, picture, signs, noises, fonts (e.g., to promote   highway safety or attention to one’s future self, as in virtual aging through   online programs) \\
	\hline
	Decrease Vagueness and Ambiguity &
	Decreasing   vagueness and ambiguity through the use of plain language \\
	\hline
	Attracting/Reducing Attention &
	Attracting   or reducing attention, including through drawing attention to certain product   attributes or through product placement (e.g., through cafeteria design) \\
	\hline
	Moral Suasion &
	Using   moral suasion, increasing fun, or triggering a sense of responsibility \\
	\hline
	Checklists &
	\\
	\hline
	Reducing paperwork &
	\\
	\hline
	Giving comparative information &
	To   overcome comparison friction \\
	\hline
	Structure of Evaluation &
	Jointly   rather than seperately evaluating goods/people (to help reduce   discrimination) \\
	\hline
	Visible Goals &
	Make   simple performance measures clearly visible so that people can immediately   assess their performance against a goal state (e.g., clearly displaying   manufacturing output and goals in factories is often, by itself, sufficient   to increase productivity \\
	\hline
	Argentum Ad Populum &
	A   practical use of this psychological effect in a text. \\
	\hline
	Group-Ad Populum &
	A practical use of this   psychological effect in a text. \\
	\hline
	Hyperbolic   Discounting &
	Retailers offer   financing and deferred payment for products on their e-commerce websites,   decoupling the purchase from the payment, lowering the purchase barrier, and   shortening the decision-making process \\
	\hline
	Decoupling &
	These   psychological effects are stated as being nudges themselves in {[}L045{]}   Actually {[}N075{]} \\
	\hline	Mental Accounting &
	These   psychological effects are stated as being nudges themselves in {[}L045{]} \\
	\hline
	Attentional Collapse &
	These   psychological effects are stated as being nudges themselves in {[}L045{]} \\
	\hline
	Messenger Effect &
	These   psychological effects are stated as being nudges themselves in {[}L045{]} \\
	\hline
	Image Motivation &
	These   psychological effects are stated as being nudges themselves in {[}L045{]} \\
	\hline
	Intertemporal Choice &
	These   psychological effects are stated as being nudges themselves in {[}L045{]} \\
	\hline
	Endowment Effect & Discrepancy between the goal and the expected savings of a retirement plan   are presented, so the users can adjust their savings decision to preserve the   endowment.\\
	\hline
	Hiding &
	Making   undesirable options harder to reach \\
	\hline
	Suggesting alternatives &
	Drawing   attention to occurences that might have not been considered \\
	\hline
	Throttling mindless activity &
	E.g.   a simple time buffer to reverse the action. (Holding a publication of a   Facebook post for 10 more additional seconds) \\
	\hline
	Creating friction &
	Attempt   to minimize intrusiveness while maintaining the capacity to change user's   behaviour. \\
	\hline
	Providing multiple viewpoints &
	Providing   an unbiased overview. \\
	\hline
	Decoy effect &
	Adding   an inferior alternative to make the other options seem better. \\
	\hline
	Biasing the memory of past experiences &
	Through   changing the endings of events, the memory of said event can be altered.   (e.g. changing the speed of a progress bar, reducing workload at the   end) \\
	\hline
	Placebos &
	Same   as placebo effect. \\
	\hline
	Deceiptive visualizations &
	Creating   optical illusions that alter people's perception and judgements. \\
	\hline
	Invoking feelings of reciprocity &
	Based   on the reciprocity bias -\textgreater      Waitress offering a mint along with the bill received higher tips. \\
	\hline
	Make resources scarce &
	Announcing   limited seats at future events increses the probability of people commiting. \\
	\hline
	Reducing the distance &
	Reducing   forms of psychological distance. Group of nudges (Framing, Endowment effect) \\
	\hline
	Instigating empathy &
	e.g.   providing an animal that changes its state based on the behaviour of a user.
	\label{table:list-of-nudges}\\
	\caption{List of nudges}
\end{longtable}

==> list_psychological_effects.tex <==
% Changing the overall size of the table
\small

\begin{longtable}{@{}p{5cm}p{8cm}@{}}
\toprule
\textbf{Effect} & \textbf{Description} \\* \midrule
\endfirsthead
%
\multicolumn{2}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
\textbf{Effect} & \textbf{Description} \\* \midrule
\endhead
%
Framing & Drawing different conclusions from the same information, depending on how that information is presented. \\* \midrule
Status Quo Bias & The tendency to like things to stay relatively the same (see also loss aversion, endowment effect, and system justification). \\* \midrule
Social Desirability Bias (Social Norms) & The tendency, when making decisions, to favour potential candidates who don't compete with one's own particular strengths. \\* \midrule
Loss Aversion & The disutility of giving up an object is greater than the utility associated with acquiring it. (see also Sunk cost effects and endowment effect). \\* \midrule
Anchoring \& Adjustment & The tendency to rely too heavily, or "anchor", on one trait or piece of information when making decisions (usually the first piece of information acquired on that subject). \\* \midrule
Hyperbolic Discounting & Discounting is the tendency for people to have a stronger preference for more immediate payoffs relative to later payoffs. Hyperbolic discounting leads to choices that are inconsistent over time – people make choices today that their future selves would prefer not to have made, despite using the same reasoning. Also known as current moment bias, present-bias, and related to Dynamic inconsistency. A good example of this: a study showed that when making food choices for the coming week, 74\% of participants chose fruit, whereas when the food choice was for the current day, 70\% chose chocolate. \\* \midrule
Decoupling & According to Prelec and Lowenstein (found in L004), it is more difficult to evaluate the costs of purchases paid by credit card in contrast to cash, as the payment is decoupled from the consumption. As a result, the perceived costs of the decision decrease. \\* \midrule
Priming & Priming is a technique whereby exposure to one stimulus influences a response to a subsequent stimulus, without conscious guidance or intention. For example, the word NURSE is recognized more quickly following the word DOCTOR than following the word BREAD. \\* \midrule
Avalaibility Heuristic & The tendency to overestimate the likelihood of events with greater "availability" in memory, which can be influenced by how recent the memories are or how unusual or emotionally charged they may be. \\* \midrule
Sunk-cost Fallacy (Commitment) & Even though economists argue that sunk costs are no longer relevant to future rational decisionmaking, in everyday life, people often take previous expenditures, say, on repairing a car or house into their future decisions regarding those properties.(Combination of multiple effects e.g. Loss Aversion, Overoptimistic probability bias) \\* \midrule
Mental Accounting & Treating a fungible resource like money as non-fungible between purposes (borrowing money to avoid taking money from a savings account). \\* \midrule
Optimism and Overconfidence bias & 2 Effects: The tendency to be over-optimistic, overestimating favorable and pleasing outcomes (see also wishful thinking, valence effect, positive outcome bias). AND Excessive confidence in one's own answers to questions. For example, for certain types of questions, answers that people rate as "99\% certain" turn out to be wrong 40\% of the time. \\* \midrule
Attentional Collapse (Attentional Bias) & The tendency of perception to be affected by recurring thoughts \\* \midrule
Messenger Effect &  \\* \midrule
Image Motivation &  \\* \midrule
Intertemporal Choice & See hyperbolic discounting \\* \midrule
Representativeness \& Stereotypes & Expecting a member of a group to have certain characteristics without having actual information about that individual. \\* \midrule
Endowment Effect & The tendency for people to demand much more to give up an object than they would be willing to pay to acquire it. \\* \midrule
Spotlight Effect & The tendency to overestimate the amount that other people notice your appearance or behavior. \\* \midrule
Decoy Effect (Asymmetric Dominance) & The decoy effect increases an option’s attractiveness by presenting the option alongside an unattractive option no one would reasonably choose—the decoy. \\* \midrule
Scarcity Effect/Bias & People tend to perceive scarce items as more attractive or desirable. \\* \midrule
Middle-Option Bias & People presented with three or more options (ordered sequentially, as by price) tend to select the middle option. \\* \midrule
Primacy and Recency Effect & That items near the end of a sequence are the easiest to recall, followed by the items at the beginning of a sequence; items in the middle are the least likely to be remembered.{[} \\* \midrule
Default Effect & When given a choice between several options, the tendency to favor the default one. \\* \midrule
Contrast Effect & An object is perceived differently when shown in isolation than when shown in contrast to other objects. For example a $5 object might seem inexpensive next to a $11 object but expensive next to an object priced at \$1. \\* \midrule
Distinction Bias & This refers to the situation where two items are viewed as more distinct (from each other) when viewed together than when viewed separately. \\* \midrule
Risk Aversion & This refers to the tendency to prefer a certain positive outcome over a risky one despite the chance of it being more profitable (in expectation) than the certain one. \\* \midrule
Ambiguity Aversion & This phenomenon in decision making refers to a general preference for known risks rather than unknown ones. The difference between risk and ambiguity aversion is subtle. Ambiguity aversion refers to the aversion to not having information about the degree of risk involved. \\* \midrule
Decision Fatique & Although not an explicit cognitive bias, decision fatigue is a phenomenon worth exploring as it refers to the manner in which decision making deviates from the expected norm as a result of fatigue induced by long periods of decision making. \\* \midrule
Selective Perception & The tendency for expectations to affect perception. \\* \midrule
Choice Supportive Bias & The tendency to remember one's choices as better than they actually were. \\* \midrule
Confirmation Bias & The tendency to search for, interpret, focus on and remember information in a way that confirms one's preconceptions. \\* \midrule
Gambler's Fallacy & The tendency to think that future probabilities are altered by past events, when in reality they are unchanged. The fallacy arises from an erroneous conceptualization of the law of large numbers. \\* \midrule
Information Bias & The tendency to seek information even when it cannot affect action. \\* \midrule
Salience Bias & The tendency to focus on items that are more prominent or emotionally striking and ignore those that are unremarkable, even though this difference is often irrelevant by objective standards. \\* \midrule
Choice Aversion &  \\* \midrule
Diversification Bias & Because resources like money or time are limited for most individuals, they have to be allocated across different goals following some rationale.  This necessity is a gateway for cognitive biases, among them the diversification bias, that is, the tendency to divide resources by the amount of available categories and allocating them evenly. \\* \midrule
Denomination Effect & Studies have also found that a higher amount of money is spent when it appears in small units ($1 bills) than larger units ($20 bills). \\* \midrule
Hindsight Bias & Refers to the common tendency for people to perceive events that have already occurred as having been more predictable than they actually were before the events took place. As a result, people often believe, after an event has occurred, that they would have predicted, or perhaps even would have known with a high degree of certainty, what the outcome of the event would have been, before the event occurred \\* \midrule
Present Bias & See hyperbolic discounting \\* \midrule
Procrastination & ? \\* \midrule
Regression to the mean & An initial sampling bias may disappear as new, repeated, or larger samples display sample means that are closer to the true underlying population mean. ? \\* \midrule
Correspondence Bias & People are more likely to describe people’s behaviour on personality traits rather than beliefs, desires, and intentions, because the latter are not readily accessible while the former are stable and enduring \\* \midrule
Simulation heuristic & People determine the likelihood of an event based on how easy it is to picture the event mentally \\* \midrule
Conjunction fallacy & Which shows that people sometimes estimate the probability of the conjunction of two facts higher than either of the individual fact if those two facts are representative of prior beliefs. \\* \midrule
Appeal to the majority (Argumentum Ad Populum) & Accepting a certain thesis based on the mere fact that the majority of people accept it. \\* \midrule
Group-Ad Populum & Accepting a certain thesis based on the mere fact that a sepcific group of people accept it. \\* \midrule
Halo effect & Positive evaluation on a specific aspect (e.g., physical attractiveness) produces a halo which determines an extension of such an evaluation to other, unrelated, aspects. \\* \midrule
Authority bias (Argentum Ad Verecundiam) & Cases of inappropriate transfer where some theses are assumed to hold merely because the people asserting them are wrongly assumed to be authorities about a certain topic due to their achievements and fame obtained in other, unrelated, fields. \\* \midrule
Accent fallacy & Emphasis on certain parts of a sentence/visual can manipulate the actual meaning of a proposition. \\* \midrule
Peak-End Rule & Memory of past experiences is shaped by two moments: Their most intese (peak) and the last episode (end). \\* \midrule
Placebo Effect & The provision of an element that has no effect upon the individual's condition, or his environment, is able to improve her mental or physical response due to its perceived effect. \\* \midrule
Reciprocity Bias & People tend to return with an equivalent action the actions that they received from others. \\* \midrule
Commitment bias & Tendency of people to keep commitments they have made. \\* \midrule
Herd instinct bias & Tendency to replicate others' actions, even if this implies overriding own beliefs. \\* \midrule
Affect heuristic & Given that our first response to stimuli are affective, they have a strong influence on decision making. \\* \midrule
Mere Exposure Effect & Prolonged exposure of a stimulus is sufficient for increasing a predisposition and preference towards it. \\* \midrule
Decision inertia & Tendency to repeat the previous decision regardless of the consequences. Similar to status-quo bias \\* \bottomrule
\caption{List of psychological effects}
\end{longtable}

==> morphological_box.tex <==
\begin{table}[]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{|
			>{\columncolor[HTML]{F2F2F2}}p{2cm} |p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
			\hline
			\cellcolor[HTML]{D8D8D8}Dimension & \multicolumn{8}{c|}{\cellcolor[HTML]{D8D8D8}Characteristic} \\ \hline
			Choice \newline architecture tool & \multicolumn{2}{c|}{Decision information} & \multicolumn{2}{c|}{Decision structure} & \multicolumn{2}{c|}{Decision assistance} & \multicolumn{2}{c|}{Decision   affection} \\ \hline
			\cellcolor[HTML]{F2F2F2} & Translate \newline information & Make \newline information visible & Provide \newline social \newline reference point & Increase messengers reputation & Increase \newline visibility of information & Instigate emotional associations  & Use insights on human tendencies & Change   choice \newline defaults \\ \cline{2-9} 
			\multirow{-2}{*}{\cellcolor[HTML]{F2F2F2}Mechanism} & Change option-related effort & Change range or composition of options & Change \newline option \newline consequences & Provide  reminders & Facilitate   commitment &  &  &  \\ \hline
			Application domain & Health & Environment & Route \newline planning & Financial &  &  &  &  \\ \hline
			Goal & Certain \newline option should be pursued & Certain \newline option should be refrained from &  &  &  &  &  &  \\ \hline
		\end{tabular}%
		}
	\caption{Morphological Box for digital nudges in recommender systems}
	\label{table:Morphological Box}
\end{table}

==> nudges_in_future.tex <==
\begin{table}[h!t]
\scriptsize
\centering
%\begin{tabular}{p{5.65cm}p{5.65cm}}
\begin{tabular}{p{5cm}p{5cm}}
  %\textbf{Possible future mechanisms} & \textbf{Possible future mechanisms (cont.)} \\
  \hline
  Attracting attention & Moral suasion \\
  Automatic enrollment & Referring to opinion leader\\
  Deceptive visualizations & Setting defaults \\
  Decision staging & Situated \\
  Explicitly mapping  & Throttle mindless activity \\
  Instigating empathy with characters & Tutorial\\
  Just-in-time  & Understanding mapping \\
  Messenger effect & Visuals \\
  Micro-Incentives & Warning \\
  \hline
\end{tabular}
\caption{Possible directions for nudges in recommender systems}
\label{tab:future-in-recommender}
\end{table} 

==> related_mechanisms.tex <==
\begin{table}[h!t]
	\scriptsize
	\centering
	\begin{tabular}{p{5.65cm}}
		\textbf{Related nudging mechanisms} \\
		\hline
		Decoy effect  \\
		Giving comparative information  \\
		Limited time window \\
		Making resources scarce \\
		Temptation \\
		Providing an explanation \\
		\hline
	\end{tabular}
	\caption{Nudging mechanisms explored in the contest of recommender systems}
	\label{tab:related-mechanisms}
\end{table} 
